Learning Likelihoods with Conditional Normalizing Flows

Normalizing Flows (NFs) are able to model complicated distributions p(y) with strong inter-dimensional correlations and high multimodality by transforming a simple base density p(z) through an invertible neural network under the change of variables formula. Such behavior is desirable in multivariate structured prediction tasks, where handcrafted per-pixel loss-based methods inadequately capture strong correlations between output dimensions. We present a study of conditional normalizing flows (CNFs), a class of NFs where the base density to output space mapping is conditioned on an input x, to model conditional densities p(y|x). CNFs are efficient in sampling and inference, they can be trained with a likelihood-based objective, and CNFs, being generative flows, do not suffer from mode collapse or training instabilities. We provide an effective method to train continuous CNFs for binary problems and in particular, we apply these CNFs to super-resolution and vessel segmentation tasks demonstrating competitive performance on standard benchmark datasets in terms of likelihood and conventional metrics.

==> sections/metric_learning.tex <==
A function $d(x, y)$ is a metric if it satisfies the following properties:

\begin{enumerate}
    \item $d(x, y) \geq 0$, non-negativity
    \item $d(x, y) = 0$ if and only if $x = y$, identity of indiscernibles
    \item $d(x, y) = d(y, x)$, symmetry
    \item $d(x, z) \leq d(x, y) + d(y, z)$, subadditivity
\end{enumerate}

A normalizing flow with a symmetric prior can be seen as learning a metric:
\begin{equation}
    p_Y(y) = p_Z(z) \left| \frac{\mathrm{d}z}{\mathrm{d}y} \right| \qquad \text{where} \qquad z = f(y)
\end{equation}


\begin{equation}
    p_Y(y) = \mathcal{N}(f(y) | \mu, \Sigma) \left| \frac{\mathrm{d}f}{\mathrm{d}y} \right|
\end{equation}

Consider a volume preserving flow such that $\frac{\mathrm{d}f}{\mathrm{d}y} = 1$, then: 

\begin{equation}
    p_Y(y) = \mathcal{N}(f(y) | \mu, \Sigma)
\end{equation}

Let $\hat{y}(x)$ be the prediction of a neural net, and $\mu = f(\hat{y})$:

\begin{equation}
    p_Y(y) = \mathcal{N}(f(y) | f(\hat{y}), \Sigma)
\end{equation}

We write a metric:

\begin{equation}
    d(y, \hat{y}) = C - \log p_Y(y) = C - \log \mathcal{N}(f(y) | f(\hat{y}), \Sigma)
\end{equation}

And simplified:
\begin{equation}
    d(y, \hat{y}) = \frac{1}{2} (z - \hat{z})^T \Sigma^{-1} (z - \hat{z}) \qquad \text{where} \qquad z = f(y) \text{ and } \hat{z} = f(\hat{y})
\end{equation}


Non-negativity (1) is satisfied because of a constant C (equal to $- \max_y \log p_Y(y)$). Identity of indiscernibles (2) is satisfied because $f$ is bijective. Symmetry (3) because $\mathcal{N}$ is symmetric, and because $\frac{\mathrm{d}f}{\mathrm{d}y} = 1$. Subadditivity in $Y$ because measurements in $Z$ using $\mathcal{N}$ satisfy subadditivity.

If we condition the function $f$ on $x$, we get something we can view as a conditional metric:

\begin{equation}
    d\left(\left. y, \hat{y} \right| x\right) = C - \log \mathcal{N}(f(y | x) | f(\hat{y} | x), \Sigma)
\end{equation}


\section{Alternative Perspective on Metric Learning}
Let us learn a metric $d_f$ by learning an invertible embedding $f: Y \to Z$. And let us put a traditional distance metric $d$ on $Z$:

\begin{equation}
d_f(y, \hat{y}) = d(f(y), f(\hat{y})) \label{eq:metric_flow}
\end{equation}

1) $d_f$ is automatically non-negative, since $d$ is non-negative, 2) it is zero iff $y = \hat{y}$, since $d(f(y), f(\hat{y})) = 0 \implies f(y) = f(\hat{y})$, which is  satisfied for invertible flows, 3) it is automatically symmetric, and 4) it satisfies the triangle inequality since
\begin{align}
    d(f(x), f(y)) &\leq d(f(x), f(z))  + d(f(z), f(y)) \\
    \implies d_f(x, y) &\leq d_f(x, z)  + d_f(z, y),
\end{align}
which we derived, just by replacing terms using Equation \ref{eq:metric_flow}. We can convert this distance to a Boltzmann-Gibbs type distribution, through negative exponentiation, so
\begin{align}
    p(y | z, d_f) = -\frac{e^{-d_f(y, z)}}{\mathcal{Z}}; \qquad \mathcal{Z} = \int_Y e^{-d_f(y, z)} \, \mathrm{d} y.
\end{align}
For instance if $d(z, y) = \|z - y\|_2$, then $p(y | z, d)$ is a Normal distribution, and $p(y | z, d_f)$ can be implemented by mapping points from $Y$ space to $Z$ space and measuring the likelihood under.....

\dan{I do not think that volume-preservation is necessary.}

There exists a trivial solution when $d$ is minimized where everything collapses to the same point \dan{but this doesn't happen if we demand bijectivity}. To avoid this, we may want to re-normalize, or use a volume preserving flow. Now suppose (using change of variables):
\begin{equation}
\int_Y \exp(-d(y, \hat{y})) dy = \int_Z \exp(-d(z, \hat{z})) dz = C
\end{equation}

When $f$ is volume preserving, it is equivalent to learning a volume preserving normalizing flow:
\begin{equation}
p_Y(y) = p_Z(z) = \frac{1}{C} \exp(-d(z, \hat{z}))
\end{equation}

==> sections/metric_tables.tex <==
\begin{table}[ht]%
\begin{centering}
\caption{\textit{Quantitative evaluation of state-of-the art SISR methods based on PSNR/SSIM results at 4x upscaling factor. We compare per-pixel loss-based, adversarial and our proposed likelihood methods trained on the DIV2K datasets. We evaluate the predictions on transformed YCbCr color space. Best performance is shown in bold. \chr{Only show 8 bit ?} }}
\label{table: metrics_sisr}
\resizebox{\columnwidth}{!}{%
 \begin{tabular}{c c c c c c c c c c c} 
        & & \multicolumn{1}{c}{\textbf{Baseline}}  & \multicolumn{2}{c}{\textbf{Per-Pixel loss}} & \multicolumn{3}{c}{\textbf{Adversarial loss}} & \multicolumn{3}{c}{\textbf{Likelihood}}\\ \cmidrule(lr){3-3}\cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
       Test Data & s  & Bicubic & PFF & SAN & ESRGAN & DLogistic & 8bitCNF & 5bitCNF \\ [0.5ex]
     \toprule
     Set5\multirow{2}{*}{}
            &4x & 28.43 / 0.8104 & PFF & SAN & 32.60/0.9011 & dlog &30.42 / 0.8892 & 28.34 / 0.7996\\
     \midrule
      Set14 \multirow{2}{*}{}
            &4x & 26.00/0.7027 & PFF & SAN &  28.99/0.7917 & dlog & 28.27/0.8133 & 26.17 / 0.7168\\ 
     \midrule
     BSD100 \multirow{2}{*}{}
            &4x & 25.96 / 0.6675 &  PFF & SAN & 27.76 / 0.7432 &  dlog & 27.11 / 0.7282 & 25.41 / 0.67144 \\ 
     \bottomrule
\end{tabular}}
\end{centering}
\end{table}

\begin{table}[ht]%
\begin{centering}
\caption{\textit{Quantitative evaluation of state-of-the art SISR methods based on PSNR/SSIM results at 2x upscaling factor. We compare per-pixel loss-based, adversarial and our proposed likelihood methods trained on the DIV2K datasets. We evaluate the predictions on transformed YCbCr color space. Best performance is shown in bold. \chr{Either show 8 or 5bit}}}
\label{table: metrics_sisr}
\resizebox{\columnwidth}{!}{%
 \begin{tabular}{c c c c c c c c c c c} 
        & & \multicolumn{1}{c}{\textbf{Baseline}}  & \multicolumn{2}{c}{\textbf{Per-Pixel loss}} & \multicolumn{3}{c}{\textbf{Adversarial loss}} & \multicolumn{3}{c}{\textbf{Likelihood}}\\ \cmidrule(lr){3-3}\cmidrule(lr){4-5} \cmidrule(lr){6-8} \cmidrule(lr){9-11}
       Test Data & s  & Bicubic & PFF & SAN & ESRGAN & DLogistic & 8bitCNF & 5bitCNF \\ [0.5ex]
     \toprule
     Set5\multirow{2}{*}{}
            &2x & 33.66 / 0.9299 & PFF & SAN &- & dlog & 8bit & 30.76 / 0.8697\\

     \midrule
      Set14 \multirow{2}{*}{}
            &2x & 30.24 / 0.8688 & PFF & SAN & 34.23 / 0.9225 & dlog & 8bit & 28.09 / 0.8494\\

     \midrule
     BSD100 \multirow{2}{*}{}
            &2x & 29.56 / 0.8431  & PFF & SAN & 32.46 / 0.9031 & dlog & 8bit & 27.96 / 0.8457 \\
     \bottomrule
\end{tabular}}
\end{centering}
\end{table}
